Concurrency and Privacy with Payment-Channel Networks

Permissionless blockchains protocols such as Bitcoin are inherently limited in transaction throughput and latency. Current efforts to address this key issue focus on off-chain payment channels that can be combined in a Payment-Channel Network (PCN) to enable an unlimited number of payments without requiring to access the blockchain other than to register the initial and final capacity of each channel. While this approach paves the way for low latency and high throughput of payments, its deployment in practice raises several privacy concerns as well as technical challenges related to the inherently concurrent nature of payments, such as race conditions and deadlocks, that have been understudied so far. In this work, we lay the foundations for privacy and concurrency in PCNs, presenting a formal definition in the Universal Composability framework as well as practical and provably secure solutions. In particular, we present Fulgor and Rayo. Fulgor is the first payment protocol for PCNs that provides provable privacy guarantees for PCNs and is fully compatible with the Bitcoin scripting system. However, Fulgor is a blocking protocol and therefore prone to deadlocks of concurrent payments as in currently available PCNs. Instead, Rayo is the first protocol for PCNs that enforces non-blocking progress (i.e., at least one of the concurrent payments terminates). We show through a new impossibility result that non-blocking progress necessarily comes at the cost of weaker privacy. At the core of Fulgor and Rayo is Multi-Hop HTLC, a new smart contract, compatible with the Bitcoin scripting system, that provides conditional payments while reducing running time and communication overhead with respect to previous approaches.

==> approach.tex <==
% !TEX root = main.tex

\section{Proposed Solution and Challenges}
\label{sec:approach}

We divide the overall \payment cycle in three phases: escrow phase, \payment phase and cash out phase. We assume that \users 
have agreed in advance on the start time and duration for each of the phases. In the escrow phase, 
\users open payment channels with each other, effectively creating a payment channel network. During the \payment phase, \users carry out 
off chain \payments using the liquidity available in the network of payment channels. Finally, during the cash out phase, \users close their 
payment channels effectively receiving the corresponding bitcoins in the Bitcoin blockchain. In the following we informally describe each of these phases.

\subsection{The escrow phase}
Assume Alice wants to open a payment channel with Bob for a value of 1 bitcoin. For that, Alice creates a Bitcoin transaction that transfers 1 bitcoin 
from her account to a deposit account and includes such transaction in the Bitcoin blockchain. At this point, 1 bitcoin is held in escrow within the deposit. 
The deposit is defined in Bitcoin script terms such that before a predefined time $t$, the 1 bitcoin can be extracted only if Alice and Bob agree. After time $t$, 
the 1 bitcoin is sent back to Alice (i.e., refund \payment). We set up $t$ to the duration of the \payment phase. 

While the escrow phase is active, every \user proceeds as Alice, effectively creating her own payment channel. At the end of this phase, several 
payment channels are submitted to the Bitcoin blockchain, thereby creating a payment channel network. 


\subsection{The \payment phase}

In this phase, we propose to leverage a set of non-colluding computing parties to perform operations on behalf of the offline \users. In detail, first every \user 
secret shares the value of her payment channel and sends one share to each of the computing parties. 
Therefore, at this point 
a computing party knows the sender, the receiver and a share of the value for each payment channel.


At this point, there are several challenges to be addressed in order to perform \payments between two \users. In particular:

\begin{itemize}
\item \emph{Find paths.} The calculation of paths between sender and receiver is the first crucial task 
towards processing a \payment request. A natural approach is to use max-flow, 
however, currently available algorithms are inefficient in practice. Instead, it has been shown that 
the landmark routing approach outperforms max-flow in practice. We plan to leverage 
landmark routing technique in our system.

\item \emph{Calculate path liquidity.} Once a path (or a set of paths) between sender and receiver 
is found, it is necessary to calculate the amount of bitcoins that can be transacted through such path. 
However, this remains a challenge since computing parties do not have the payment channel values 
in clear. Instead, we can leverage existing Multi-Party Computation algorithms to perform such 
computation in a distributed manner.

\item \emph{Payment atomicity.} In order to ensure integrity of \payments, in other words, to ensure that 
no honest \user incurs in money loss, payments must be atomic: either every channel in the path is used 
or the \payment is not executed. In order to achieve such property, we plan to define a smart contract 
based in the currently available Bitcoin script. Designing the specific terms of such contract remains a challenge.
\end{itemize}



\subsection{Cash out phase}
Once the payment phase is finished, the computing parties can exchange their shares of the state 
for each payment channel and thereby reconstruct their final values.  Then, both users associated 
to a given payment channel 
can propagate their agreements with the final channel value to the Bitcoin blockchain and 
the payment channel will be effectively closed. 

In this phase there are open challenges to be addressed as well. In particular, certain \users or computing 
parties can decide not to follow the protocol and act arbitrarily instead. In order to handle such 
case, we plan to define an accountability mechanism that creates a proof of misbehavior by a 
certain \user. Additionally, we plan to define a smart contract to punish a misbehaving \user when 
a misbehavior proof is generated.




==> concurrency.tex <==
% !TEX root = main.tex
\section{Concurrency Analysis}
\label{sec:concurr}
%

In this section, we describe a \emph{transactional} protocol for concurrent \payments
that provides \emph{atomic} \pay operations (\`a la \emph{serializability}~\cite{Pap79-serial}). 
As discussed in~\cref{sec:atomic-payments}, intuitively a \pay operation must ensure that 
either the capacity of all \pcs in the path are updated or none of the \pcs is changed.

%We state the following trivial lower bound on the failure resilience
%of any concurrent transactional protocol for \pcns and we include the proof in~\cref{sec:concurr}. 





%A \payment can be aborted due to several reasons. First,  
%(i.e., another \payment already got the lock) along the 
%path. Such abortion triggers a $\release(\pid)$ message that gets propagated from 
%the conflicting link back to the sender through the path, thereby (possibly) releasing 
%the locks associated to \payment $\pid$. Once the $\release(\pid)$ message 
%reaches the sender, she can retry it again after a randomly chosen delay.
%
%Second, the \payment $\pid$ reaches the receiver. Then, the receiver starts 
%a $\confirm(\pid)$ message that gets propagated towards the sender through 
%the \pcs in the payment path.  Once the sender receives the $\confirm(\pid)$ message, 
%she knows that it has been successful and terminates. Moreover, the $\confirm(\pid)$ 
%releases the all the locks associated to $\pid$ in the path, thereby ``freeing'' the path 
%for further \payments. 
%


% \begin{definition}[Safety]
% %  If the assumptions on the communication model hold and there exists 
% % a total ordering between the \payments and the \users, then the outcome of a \payment 
% % (i.e., successfully completed, unsuccessfully completed or aborted) must be the same 
% % for all \pcs along the \payment path.
% \end{definition}
%



%

% \TODOP{Here a good argument is that once a \payment reaches confirm (and one 
% for sure does because is the biggest), the confirm message wins over everything 
% in its way back to the sender}
% 
% 
% 
% \TODOP{What are the privacy implications of this protocol for concurrent \payments}
% 
% \TODOP{Add argument about overhead of the concurrency protocol}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> draft-notes.tex <==
% !TEX root = main.tex

\section{Comparison between Bitcoin Payment Channels and our work on credit networks}

\def\arraystretch{1.5}
\begin{tabular} {p{2cm} | p {6cm} | p{6cm}}
& Payment Channels & Credit Network (SilentWhispers)\\
\hline
Network Topology & 
	\textbf{Publicly available:} Every pair of \users create the link by creating a 2 out 2 escrow transaction in Bitcoin.  &
	\textbf{Unknown:} The existence of a link between two \users is only known to those \users\\
\hline
Assumption on \users & 
	\textbf{No gateways:} Any \user can create a channel with any other \user. There is no concept of gateway &
	\textbf{Gateways:} There are highly connected \users in the network. They are used in most of the payment paths.\\
\hline
Arbitrator & 
	\textbf{The Bitcoin rules:} The Bitcoin protocol defines a set of rules that can be used in case of dispute. Limited set of rules\footnote{
	Bitcoin scripts can only be used to perform two cryptographic operations: (1) validate the preimage of a hash, or (2) validate an ECDSA signature on a 
	Bitcoin transaction~\cite{tumblebit}}. & 
	\textbf{A third party (e.g., judge):} Define its own arbitrator to solve disputes. More flexibility.\\
\hline
Current Link State &
	\textbf{Defined by Bitcoin rules:} The limited set of rules in Bitcoin determine whether a given state of the link is valid (e.g., signature on the 
	transaction in the \emph{clear} from both \users sharing the link.)&
	\textbf{Defined by the protocol: } A protocol-defined state crafted for this purpose.
	\\
\hline
Threat Model &
	\textbf{No trusted \user/server:} An attacker can control an arbitrary number from all \users and thus an arbitrary number of channels &
	\textbf{Non-colluding gateways:} An attacker controls arbitrary number of \users and links. However, there exists a set of well-known non-colluding gateways.\\
\hline
\end{tabular}





\newpage
\section{Comparison between different works on Bitcoin payment channels}
\def\arraystretch{1.5}
{\small 
\begin{tabular} {c | c | c | c | c }
 & Lightning Network~\cite{ln} & TumbleBit~\cite{tumblebit} & Flare~\cite{flare} & Bolt~\cite{bolt} \\
 \hline
 Channel Direction & 
 	Bidirectional &
	Unidirectional & 
	Bidirectional &
	Bidirectional\\
\hline
Bitcoin Compatibility &
	Yes &
	Yes &
	 Yes &
	 No\\
\hline 
\multirow{2}{*}{Privacy notion} &
	None &
	Unlinkability &
	sender-receiver anon&
	Payment anonymity\\

	&
	&
	payer-payee&
	&
	Balance\\	
\hline
Multihop defined&
	Yes &
	No\footnote{It is defined as a single hop payment. It is not clear how to make it multihop: Who has the solution to the puzzle and when to reveal it?} &
	Yes &
	No\footnote{As in TumbleBit is not defined for multihop. Not clear how to make it in practice}\\
\hline 
Variable amount &
	Yes &
	Fixed &
	Yes &
	Yes\\
\hline
Online \users required&
	Yes &
	Yes &
	 Yes &
	Yes\\
\hline	
%DoS and Sybil protection &
%	& 
%	Fees &
%	&
%	\\
\end{tabular}
}
\subsection{Questions}
\begin{itemize}
 \item It is possible to have a bidirectional channel between two \users or alternatively two unidirectional channels, one on each direction. What is the better approach? 
 (Think of fees and bitcoins being locked)
\end{itemize}

\section{Notes on challenges}
Related works~\cite{tumblebit, bolt, ln, flare} require that \users in the payment path are online. It would be interesting to have a scheme that allows to perform payments where only 
payer and payee are online.

Related work considers providing any privacy notion by having only one intermediate \user in the payment path. 
One of the challenges is to ensure \textbf{atomic payments} with more than one intermediate, offline \user. 


\subsection{Challenges to overcome towards a solution}
Let assume that there exists a set of non-colluding servers. They can execute MPC protocols (either using a threshold decryption scheme or a secret sharing scheme). 
One point here is that servers should not learn anything else than what is publicly available in the blockchain. 

We can think of the system working in epochs. At the beginning of the epoch, a server reconstructs the complete network composed by payment channels in the 
blockchain and at the end of the epoch these channels are closed. Moreover, each \user gives each server a ``share'' (e.g., encryption of the value) of the payment channel value. This share 
can be used to perform MPC operations. 

The following functionalities might be required:

\begin{enumerate}
\item \emph{Routing: Find paths between payer and payee.} Possibly apply landmark routing using nodes with high degree as landmarks. 

\item \emph{Calculate credit available in a path.} Possibly use an MPC  protocol for min computation

\item \emph{Perform payment over a path.} There are some challenges here:
	\begin{itemize}
		\item \emph{Ensure that the path has enough credit.} Possibly use a Less Than Zero MPC protocol.
		\item \emph{Perform the payment atomically.} Here we cannot use signatures of a ``temporal state'' as in SilentWhispers, since that is already a valid state. 
		Possibly use pay to hash script function.
		\item \emph{Who signs the link states for each payment?} Possibly, each \user shares her signing key among the servers so that they can jointly create 
		a signature. Nevertheless, how to ensure that servers do not sign transactions without the \user consent? Assume honest majority of servers?
		\item \emph{How to hide the value?} A new link state is only valid if the transaction in the clear is signed by both \users sharing the channel.
		
	\end{itemize}
\end{enumerate}



\section{Towards a solution}
\subsection{Online \users}
Here we assume that the network of payment channels is public and \users can find payment paths on their own. Nevertheless, we need to argue how 
\users get the complete network in the first place:
\begin{itemize}
\item Each \user could be a Bitcoin full node (i.e., each \user has a copy of the whole blockchain). This might be unrealistic
\item Each \user queries a full node for the complete network (i.e., using the Bitcoin thin client mechanism)
\end{itemize}


Once the payment path is known, we need to perform an atomic payment from sender to receiver hiding the value that is transacted. One possibility is 
to perform the transaction using Confidential Transactions~\cite{ct-bitcoin} already available in Bitcoin. However, this is defined for a single hop payment, not 
for a multi-hop payment. The challenge is:
\begin{itemize}
\item If a \user receives a commitment of the transaction value from her previous neighbor in the path, who does the \user know that she has enough 
credit on her link for that transaction?

\item Confidential transactions in Bitcoin define already a range proof. We might be able to leverage that. 
\end{itemize}


\subsection{Offline \users}


==> dtlc.tex <==
% !TEX root = main.tex

\section{Discrete-Log Time Lock Contracts} 
\label{sec:dltc}
\TODOP{Think where to integrate this part}



To improve the scalability of our system, we propose a variant of HTLC that we call
Discrete-Log Time Lock Contracts (DTLC). Our solution leverages the
homomorphic properties of cyclic groups of prime order to generate
unlinkable smart contracts. DTLC allows groups of users to perform
anonymous payments without sacrificing atomicity at a very small cost.
The message flow of our algorithm is depicted in Figure~\ref{fig:pay}.
More specifically, the challenge issued by the receiver is of the form
$X = g^x \in \GG$, for some random $x \in \ZZ_p$, which is propagated
(starting from the sender) through the transaction path. Upon
receiving $X$ each user $\uid_i$ forwards it to the next node in the
path $\uid_{i+1}$, who replies with a random element $z \in \ZZ_p$.
Then the user generates the following smart contract $\gamma_{\uid_i, \uid_{i+1}}$:

\begin{center}
\small
\vspace{-1em}
\resizebox{\columnwidth}{!}{
\fbox{
\parbox{\columnwidth}{
{\bf DTLC ($\uid_i$, $\uid_{i+1}$, $Z'$, $\val$, $t'$):}
\begin{asparaenum}
\item If $\uid_{i+1}$ produces $z'$ such that $g^{z'} = Z'$ before $t$
  days, $\uid_i$ pays $\uid_{i+1}$ $\val$ bitcoins.
\item If $t'$ days elapse, $\uid_i$ gets back $\val$ bitcoins.
\end{asparaenum}
}}}
\end{center}

Where $Z'$ is defined as $Z' = X \cdot g^z$. Note that the user
$\uid_i$ should only generate a DTLC if the previous user in the path
provided him with a well-formed DTLC for the same amount $\val$. Also,
as discussed before, the time $t'$ of the contract between $\uid_i$
and $\uid_{i+1}$ should exceed the time $t$ of the contract between
$\uid_i$ and $\uid_{i-1}$. If all of the above conditions are met,
correctness is easy to check: In order to unlock the DTLC,
$\uid_{i+1}$ must provide a solution $z' = x + z$. Therefore $\uid_i$
can infer the value of $x$ and unlock the contract with $\uid_{i-1}$,
pulling the same amount $\val$. Note that this chain of events can
only be started when the receiver releases the value of $x$, thereby
confirming that she received the correct transaction value. Unlocking a
contract without the help of the receiver is as hard as breaking the
discrete logarithm problem over $\GG$.

One can easily see that each contract encodes a problem relative to a
group element ($g^{x+z}$ in the former example) which is uniformly
distributed over $\GG$. This makes contracts belonging to the same
payments no longer linkable. Clearly, this extension still leaks the
value of the value $\val$, which could potentially lead to privacy
attacks when a \pc is closed. 
A possible solution consists on the  use of confidential transactions 
to close the \pc while hiding  the
corresponding value $\val$ (see~\cref{sec:ct}). 
%However, we can also
%imagine that two honest users would seldom upload DTLCs to the
%blockchain, using them rather as an insurance of correctness of the
%payment.  
On the downside, DTLC sacrifice the compatibility of
\sysname with Bitcoin (although cryptocurrencies with a complete scripting
language, like Etherem~\cite{raiden-nw}, can still support it), since the
Bitcoin script language does not currently support modular arithmetic for
large numbers. However, we argue that our proposed modifications 
are conceptually simple and computationally efficient, so
the Bitcoin community might consider to implement it in the near future.

\begin{figure}[t]
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm,semithick, transform shape, scale=0.8, baseline]   
 \tikzstyle{probabilistic}=[rectangle, rounded corners, fill=white,text=black, draw=black, minimum size=0.3cm,  transform shape]
 \tikzstyle{markovian}=[rectangle,text=black, draw=black, transform shape]
 \tikzstyle{none}=[draw=none,fill=none,inner sep=0,outer sep=0]
 \tikzstyle{reward}=[draw=none,fill=none,inner sep=0,outer sep=0]
 
 \node[markovian, minimum width=3cm, minimum height = 4cm] (midrec)
 {$\begin{array}{l}Check \\ \contract_{\uid_{i-1}, \uid_i}(g^{x+y}, \val, t)\end{array}$};

 \node[none] (user) at($(midrec)+(0, +2.6cm)$) {\underline{$\uid_i$}};
 \node[none] (user) at($(midrec)+(-3.7, +2.6cm)$) {\underline{$\uid_{i-1}$}};
 \node[none] (user) at($(midrec)+(+3.7, +2.6cm)$) {\underline{$\uid_{i+1}$}};

 \node[none] (text) at($(midrec)+(0, +1.35cm)$) {$y \gets \ZZ_p$};
 \node[none] (text2) at($(midrec)+(0, -1.35cm)$) {$\begin{array}{l}Generate \\ \contract_{\uid_{i}, \uid_{i+1}}(g^{x+z}, \val, t')\end{array}$};

 \node[none] (lar1) at($(midrec)+(-4cm,1.9)$) {};  
 \node[none] (lare1) at($(midrec)+(-1.5cm,1.9)$) {};  

 \node[none] (lare2) at($(midrec)+(-4cm,1.2)$) {};  
 \node[none] (lar2) at($(midrec)+(-1.5cm,1.2)$) {};  

 \node[none] (lar3) at($(midrec)+(-4cm,0.5)$) {};  
 \node[none] (lare3) at($(midrec)+(-1.5cm,0.5)$) {};  

 \node[none] (lare4) at($(midrec)+(+4cm,-0.5)$) {};  
 \node[none] (lar4) at($(midrec)+(+1.5cm,-0.5)$) {};  

 \node[none] (lar5) at($(midrec)+(+4cm,-1.2)$) {};  
 \node[none] (lare5) at($(midrec)+(+1.5cm,-1.2)$) {};  

 \node[none] (lare6) at($(midrec)+(+4cm,-1.9)$) {};  
 \node[none] (lar6) at($(midrec)+(+1.5cm,-1.9)$) {};
 
 \path
 (lar1) edge [midway] node {$(g^x, \val)$} (lare1)
 (lar2) edge [above,midway] node {$y$} (lare2)
 (lar3) edge [above,midway] node {$\contract_{\uid_{i-1}, \uid_i}(g^{x+y}, \val, t)$} (lare3)
 (lar4) edge [above,midway] node {$(g^x, \val)$} (lare4)
 (lar5) edge [above,midway] node {$z$} (lare5)
 (lar6) edge [above,midway] node {$\contract_{\uid_{i}, \uid_{i+1}}(g^{x+z}, \val, t')$} (lare6)      
;
\end{tikzpicture}
\caption{Message flow of our extension}
\label{fig:pay}

\end{figure}





\TODOP{Can public fees be used to break sender/receiver anonymity? Idea: use similar fees\\
Can the correlated timeout for the channels break anonymity? }


==> extensions.tex <==
% !TEX root = main.tex
%\section{Protocol Extensions}
%\label{sec:system-extensions}
%
%
%In this section, we describe extensions to \sysname to improve upon
%privacy issues when closing a \pc and logging its state in the publicly available blockchain 
%as well as with the
%HTLC contract used in the \pay operation.


\section{Confidential Transactions and \pcns}\label{sec:ct}
\TODOP{Say that Confidential Transactions are only defined for Bitcoin today}

Currently, opening a new \pc requires to publish a Bitcoin transaction 
in the blockchain that publicly  
reveals not only the two \accs that share the \pc but, most importantly, 
the initial \capacity of the \pc. Similarly, closing a \pc also requires to add a 
Bitcoin transaction in the blockchain that trivially reveals the final \capacity 
distribution in the \pc. At a large scale, current opening and closing of \pcs 
reveal who pays what to whom in an aggregated form. 


Although revealing the counterparties in a \pc is an inherent assumption not only 
in this work but also in other currently proposed \pcns, the initial and final \capacity 
of a \pc needs to be disclosed only to \pc counterparties. To achieve that, it is possible to 
leverage Confidential Transactions (CT)~\cite{ct, ct-investigation}, a modified Bitcoin transaction 
where the \payment amounts are visible only to the sender and receiver of a Bitcoin 
\payment. 

In a nutshell, a CT includes amounts in the form of commitments, a cryptographic construction 
the ensures the confidentiality of the committed values (i.e., hiding property) from \users other than 
sender and receiver. Moreover, additive homomorphic property of the commitment scheme allows 
any \user to verify that the sum of input committed values is equal to the sum of output committed 
values. Additionally, the inclusion of a cryptographic proof of that each committed value is in a range 
$0, \ldots, 2^n$ (i.e., intuitively proving that all committed amounts are positive) 
ensures that  no new coins are created in the transaction. We refer the reader 
to~\cite{ct, ct-investigation} for further details. 

The CT can be used to improve the privacy on the management of \pc as follows. A pair of 
\users open a \pc by publishing a CT. As the CT reveals the initial committed \capacity of the 
channel to both \users, they can use this value locally to adjust it according to \payments 
routed through their channel in the \pcn. Finally, when \users are about to close the \pc, they 
can collaborate to create a new CT (instead of a plain Bitcoin transaction). Again, both counterparties 
can verify that the channel is correctly closed with the correct distribution of coins, while maintaining 
those amounts hidden to the rest of \users. 
\TODOP{It is possible that \users do not want to collaborate. Two solutions: still close the channel in 
plain, or force to have each partial state of the channel encoded as a CT (however, CT is 
way bigger than normal transaction}











%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> macro.tex <==

\newcommand{\td}{\ensuremath{\mathsf{td}}}
\newcommand{\hc}{\ensuremath{\mathsf{hc}}}
\newcommand{\expHC}{\ensuremath{\mathsf{HC}}}
\newcommand{\URL}[1]{{\color{blue}{\url{#1}}}}
\newcommand{\nizk}{\ensuremath{\mathsf{NIZK}}\xspace}
\newcommand{\setup}{\ensuremath{\mathsf{Setup}}\xspace}
\newcommand{\crs}{\ensuremath{\mathsf{crs}}\xspace}
\newcommand{\com}{\ensuremath{\mathsf{com}}\xspace}
\newcommand{\decom}{\ensuremath{\mathsf{decom}}\xspace}
\newcommand{\comV}{\ensuremath{\mathsf{V}_\mathsf{com}}\xspace}
\newcommand{\comP}{\ensuremath{\mathsf{P}_\mathsf{com}}\xspace}
\newcommand{\prover}{\ensuremath{\mathsf{P}}\xspace}
\newcommand{\verifier}{\ensuremath{\mathsf{V}}\xspace}
\newcommand{\Client}{\ensuremath{\mathsf{Client}}\xspace}
\newcommand{\Server}{\ensuremath{\mathsf{Server}}\xspace}
\newcommand{\Attacker}{\ensuremath{\mathsf{Attacker}}\xspace}
\newcommand{\client}{\texttt{Client}}
\newcommand{\auth}{\texttt{Authority}}
\newcommand{\dataown}{\texttt{DataOwner}}
\newcommand{\server}{\texttt{server}}
\newcommand{\attacker}{\texttt{attacker}}
\newcommand{\BookURL}{{\color{blue}{\bookurl}}}
\newcommand{\hint}[1]{({\bf Hint}: \textit{#1})}
\newcommand{\Mac}{\ensuremath{\mathsf{Mac}}}
\newcommand{\bit}[1]{\{0,1\}^{#1}} 
\newcommand{\xor}{\oplus}
\newcommand{\group}[2]{\left(#1,#2\right)}
\newcommand{\bi}{\ensuremath{\mathsf{b}}}
\newcommand{\Setup}{\ensuremath{\mathsf{Setup}}}
\newcommand{\enc}{\ensuremath{\mathsf{Enc}}}
\newcommand{\eval}{\ensuremath{\mathsf{Eval}}}
\newcommand{\keygenenc}{\ensuremath{\mathsf{KeyGenE}}}
\newcommand{\keygensig}{\ensuremath{\mathsf{KeyGenS}}}
\newcommand{\sig}{\ensuremath{\mathsf{Sign}}}
\newcommand{\ver}{\ensuremath{\mathsf{Verify}}}
\newcommand{\dec}{\ensuremath{\mathsf{Dec}}}
\newcommand{\pk}{\ensuremath{\mathsf{pk}}}
\newcommand{\ek}{\ensuremath{\mathsf{ek}}}
\newcommand{\vk}{\ensuremath{\mathsf{vk}}}
\newcommand{\dk}{\ensuremath{\mathsf{dk}}}
\newcommand{\sk}{\ensuremath{\mathsf{sk}}}
\newcommand{\HH}{\ensuremath{\mathsf{H}}}
\newcommand{\msk}{\ensuremath{\mathsf{msk}}}
\newcommand{\msg}{\ensuremath{\mathsf{m}}}
\newcommand{\cipher}{\ensuremath{\mathsf{c}}}
\newcommand{\aaa}{\ensuremath{\mathsf{A}}}
\newcommand{\KeyGen}{\ensuremath{\mathsf{KeyGen}}}
\newcommand{\GroupGen}{\mathcal G}
\newcommand{\GG}{\ensuremath{\mathbb{G}}}
\newcommand{\NN}{\ensuremath{\mathbb{N}}}
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\UU}{\ensuremath{\mathbb{U}}}
\newcommand{\AAA}{\ensuremath{\mathbb{A}}}
\newcommand{\CC}{\ensuremath{\mathcal{C}}}
\newcommand{\FF}{\ensuremath{\mathcal{F}}}
\newcommand{\MM}{\ensuremath{\mathcal{M}}}
\newcommand{\set}[1]{\ensuremath{\{#1\}}\xspace}
\newcommand{\prob}[1]{\ensuremath{\mathsf{Pr}\left[#1\right]}\xspace}
\newcommand{\sd}[1]{\ensuremath{\mathsf{SD}\left[#1\right]}\xspace}
\newcommand{\negl}{\ensuremath{\mathsf{negl}}}
\newcommand{\advan}{\ensuremath{\mathbf{Adv}}}
\newcommand{\adv}{\ensuremath{\mathcal{A}}}
\newcommand{\red}{\ensuremath{\mathcal{R}}}
\newcommand{\pp}{\ensuremath{\mathsf{PP}}\xspace}
\newcommand{\ppt}{\ensuremath{\mathsf{PPT}}\xspace}
\newcommand{\poly}{\ensuremath{\mathsf{poly}}\xspace}
\newcommand{\cheat}{\ensuremath{\mathsf{cheat}}\xspace}
\newcommand{\si}{\ensuremath{\mathsf{S}}}
\newcommand{\pay}{\ensuremath{\mathsf{pay}}\xspace}
\newcommand{\test}{\ensuremath{\mathsf{test}}\xspace}
\newcommand{\relation}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\language}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\prover}{\ensuremath{\mathsf{P}}\xspace}
\newcommand{\verifier}{\ensuremath{\mathsf{V}}\xspace}


\newtheorem{assumption}{Assumption}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% TeX-PDF-mode: t 
%%% End: 

==> routing-algorithms.tex <==
% !TEX root = main.tex

\section{Comparison of Possible Routing Strategies}

\begin{table*}
\centering
\begin{tabular}{c | c | c}
\hline
 & Onion Routing & \sysname\\
 \hline
 Message Integrity & HMAC & None (not required in our specific application. Save in size)\\
 Privacy properties & users don't know if they are in the same path & users know if they are  in the same path\\
 TLS channels & not required & required\\
\end{tabular}
\end{table*}

==> security-analysis.tex <==
% !TEX root = main.tex


\section{Security Analysis}
\label{sec:sec-analysis}

We hereby state the privacy results for \sysname and defer the 
security proofs to~\cref{sec:security-proofs}.

\begin{theorem}[Value Privacy]\label{thm:valpri}
  Let $\Pi^\mathsf{PKE}$ be a chosen ciphertext secure public-key
  encryption scheme, and let $\Pi^\mathsf{DS}$ be an existentially
  unforgeable digital signature scheme. Then \sysname is value
  private.
\end{theorem}



\begin{theorem}[Test Privacy]\label{thm:testpri}
  Let $\Pi^\mathsf{PKE}$ be a chosen ciphertext secure public-key
  encryption scheme, and let $\Pi^\mathsf{DS}$ be an existentially
  unforgeable digital signature scheme. Then \sysname is test private.
\end{theorem}



\begin{theorem}[Anonymity]\label{thm:anon}
  Let $\Pi^\mathsf{PKE}$ be a chosen ciphertext secure and key-private
  public-key encryption scheme, and let $\Pi^\mathsf{DS}$ be an
  existentially unforgeable digital signature scheme. Then \sysname is
  anonymous.
\end{theorem}



==> security-proofs.tex <==
% !TEX root = main.tex

\section{Formal Results and Security Proofs}
\label{sec:security-proofs}


In this section we formally define the security and privacy properties
of a Payment Channel Network and we prove that \sysname achieves
them.

\subsection{Value Privacy}

Value privacy says that the adversary cannot distinguish between any
two transactions performed by a honest node. To make the game
non-trivial we have to enforce that, if some corrupted node lies in
the path of the two payments, then the two transacted values shall be
the same: Otherwise an adversary could easily distinguish between the
two cases by checking the balance of her links. Additionally, after
the challenge transaction we perform a \emph{balancing transaction} to
avoid trivial attacks where the adversary just checks the status of
the network after the payment has been processed. As discussed
in~\cite{privpay-ndss}, the balancing transaction models the
uncertainty due to the continuous operations happening in the
network. The formal definition follows.

\begin{definition}[Value Privacy]\label{def:valpri}
  We say that a scheme achieves \emph{value privacy} if for all
  $\lambda \in \NN$ and for all probabilistic-polynomial time adversaries $\adv$
  there exists a negligible function such that the success probability
  of $\adv$ in the following experiment is negligibly close to
  $\frac{1}{2}$.
  \begin{asparaitem}
  \item[] \textbf{Setup:} In the setup phase the public parameters
    $\pp$ of the system are initialized and the adversary is provided
    with the tuple $(1^\lambda, \pp)$.
  \item[] \textbf{Phase 1:} In this phase the adversary can spawn
    arbitrary many users of the system and adaptively corrupt any
    subset of them. Upon corruption the adversary receives the
    (static) internal state of the honest clients. From the moment of
    the corruption of a client $c$, every message to $c$ is routed to
    the adversary and the adversary is allowed to send arbitrary
    messages on behalf of $c$. The experiment maintains as a state
    lists of all the corrupted and honest clients (denoted by
    $\mathcal{C}$ and $\mathcal{H}$, respectively) and of the internal
    state of the honest clients. Additionally, the adversary has
    access to the following interfaces:
    \begin{itemize}
    \item $\test((c_1, \dots, c_n),\val)$: On input a set of clients $(c_1,
      \dots, c_n)$ and a value $\val$, the challenger executes a $\test$ operation on the
      same inputs, impersonating the honest clients.
    \item $\pay((c_1, \dots, c_n), v)$: On input a set of clients
      $(c_1, \dots, c_n)$ and a value $\val$, the challenger executes a
      $\pay$ operation on the same inputs, impersonating the honest
      clients.
    \end{itemize}
  \item[] \textbf{Challenge:} The adversary outputs a tuple $((c_1^*,
    \dots, c_m^*),$ $(v_0, v_1), u)$. If there exists a client $c^*_i
    \in \mathcal{C}$, then we require that $\val_0 = \val_1$. The challenger
    than flips a bit $b \in \{ 0,1\}$ and executes the $\pay$
    operation on inputs $((c_1^*, \dots, c_m^*), v_b)$, impersonating
    the honest clients. If the operation is successful, the balancing
    transaction is defined as $\pay((c_1^*, \dots, c_m^*), u - v_b)$,
    otherwise is $\pay((c_1^*, \dots, c_m^*), u)$. The challenger
    executes the balancing transaction impersonating the honest
    clients. If the balancing transaction fails, the challenger
    aborts.
  \item[] \textbf{Phase 2:} The adversary has access to the same
    interfaces as in phase 1 except that she can no longer corrupt
    honest clients that belong to the challenge set.
  \item[] \textbf{Output:} The adversary outputs a bit $b'$ and the
    challenger returns $b = b'$.
  \end{asparaitem}
\end{definition}

\subsection{Test Privacy}

Test privacy requires that the test operation does not reveal any
additional information beyond its output, i.e., the issuer of a
request just learns whether the credit of a given path is enough to
transact a certain value $\val$. Note that any two (possibly
malicious) users can run the $\test$ algorithm for any possible path
of users that connects them. Therefore, there is no point in hiding
this information, which is inherently leaked by the
functionality. Instead what we would like to achieve is that $\test$
is securely computed over paths of contiguous honest users. This is
modeled as a classical indistinguishability notion for secure
computation in the following. \NEWPfor{SGAM}{170216}{We describe only the changes 
with respect to~\cref{def:valpri}.}

\begin{definition}[Test Privacy]\label{def:testpri}
  We say that a scheme achieves \emph{test privacy} if for all
  $\lambda \in \NN$ and for all probabilistic-polynomial time adversaries $\adv$
  there exists a negligible function such that the success probability
  of $\adv$ in the following experiment is negligibly close to
  $\frac{1}{2}$.
  \begin{asparaitem}
  %\item[] \textbf{Setup \& Phase 1:} See Definition~\ref{def:valpri}.
  %\item[] \textbf{Phase 1:} See Definition~\ref{def:valpri}.
  \item[] \textbf{Challenge:} The adversary outputs a tuple
    $(\sender,\receiver, (c_1^*, \dots, c_m^*),$ $(w_0^0, \dots, w_m^0),
    (w_0^1, \dots, w_m^1), \val)$. The challenger flips a fair coin $b
    \in \{0,1\}$. If $\sender \in \mathcal{C}$ or $\receiver \in
    \mathcal{C}$ we require that 
    \REPLACEPfor{SGAM}{170216}{\[
    \mathrm{min}\{ w_i^0\}_{i\in[m]} \stackrel{?}{<} \val \REPLACEPfor{SGAM}{170216}{\implies}{=}
    \mathrm{min}\{ w_i^1\}_{i\in[m]} \stackrel{?}{<} \val.
    \]}{$\mathrm{min}\{ w_i^0\}_{i\in[m]} \stackrel{?}{<} \val$  iff $\mathrm{min}\{ w_i^1\}_{i\in[m]} \stackrel{?}{<} \val$.}
  We distinguish four cases:
  \begin{asparaenum}
  \item $(\sender, \receiver) \in \mathcal{C}^2$: The attacker provides the first message
      of a $\test$ query on input $\val$ on behalf of $\sender$, then the
      challenger simulates the intermediate users using link values
      $(w_0^b, \dots, w_m^b)$, respectively. If any of the
      intermediate users (except for the receiver $\receiver$) belongs to
      $\mathcal{C}$, then the challenger aborts.
    \item $\sender \in \mathcal{C}$: Same as above except that the
      challenger also checks whether $\receiver \in \mathcal{H}$ and
      aborts if this is not the case.
    \item $\receiver \in \mathcal{C}$: The challenger generates a $\test$
      query on inputs $(c_1^*, \dots, c_m^*)$ and $\val$ and simulates
      the honest users using link values $(w_0^b, \dots, w_m^b)$,
      respectively. If there exists an $i \in [m]: c_i^* \in
      \mathcal{C}$, then the challenger aborts.
    \item $(\sender,\receiver) \in \mathcal{H}^2$: The challenger
      generates a $\test$ query on inputs $(c_1^*, \dots, c_m^*)$ and
      $\val$ and simulates the honest users using link values $(w_0^b,
      \dots, w_m^b)$, respectively. If, for all $i \in [m]$ and for
      all $j \in [m]$ such that $i\le j$, there exists a sequence
      $(c_i^*, \dots, c_j^*) \in \mathcal{H}^{1+j-i}$ such that
      $(c_{i-1}^*, c_{j+1}) \in \mathcal{C}^2$ (i.e., there exists an
      interrupted sequence of corrupted clients), then the challenger
      aborts.
    \end{asparaenum}
  %\item[] \textbf{Phase 2 \& Output:} See Definition~\ref{def:valpri}.
  %\item[] \textbf{Output:} See Definition~\ref{def:valpri}.
  \end{asparaitem}
\end{definition}

\subsection{Anonymity}

We collapse the notions of sender and receiver
privacy~\cite{privpay-ndss, silentwhispers} into a single definition
of anonymity. In a nutshell, anonymity guarantees that the
intermediate nodes of any transaction cannot guess identify the sender
and the receiver. In our indistinguishability notion we constrain the
two challenge sets to avoid trivial attacks: Clearly we cannot hide to
the eyes of a corrupted user whether she took part in a transaction or
not. Also, any user always learns the neighbours that she exchange
messages with (the previous and the next hop in the transaction
path). The property is formalized below. \NEWPfor{SGAM}{170216}{We describe only the changes 
with respect to~\cref{def:valpri}.}

\begin{definition}[Anonymity]\label{def:anon}
  We say that a scheme achieves \emph{anonymity} if for all $\lambda
  \in \NN$ and for all probabilistic-polynomial time adversaries
  $\adv$ there exists a negligible function such that the success
  probability of $\adv$ in the following experiment is negligibly
  close to $\frac{1}{2}$.
  \begin{asparaitem}
  %\item[] \textbf{Setup \& Phase 1:} See Definition~\ref{def:valpri}.
  %\item[] \textbf{Phase 1:} See Definition~\ref{def:valpri}.
  \item[] \textbf{Challenge:} The adversary outputs a tuple $((C^0
    =(c_1^*, \dots, c_{m'}^*), C^1 =(c_{m'+1}^*, \dots, c_m^*)), v,
    \op \in \{ \test, \pay\})$.  For such a tuple to be admissible we
    require that $(c_1^*, c_{m'+1}^*) \in \mathcal{H}^2$. For all
    clients $c^* \in \mathcal{C}$ we additionally require that if $c^*
    \in C^0$ then $c_i^* \in C^1$, and vice versa. Let $j$ and $k$ be
    the indices such that $c^* = c_j^* \in C^0$ and $c^* = c_k^* \in
    C^1$, we also require that $c_{j-1}^* = c_{k-1}^*$ and $c_{j+1}^*
    = c_{k+1}^*$.  The challenger than flips a bit $b \in \{ 0,1\}$
    and executes the operation $\op$ on inputs $(C^b, v)$,
    impersonating the honest clients. If $\op = \pay$ and $\pay(C^b,
    v)$ was successful, then the challenger executes the balancing
    transaction by running $\pay$ on $(C^{1\oplus b}, v)$,
    impersonating the honest clients. If the balancing transaction is
    not successful, then the challenger aborts.
  %\item[] \textbf{Phase 2 \& Output:} See Definition~\ref{def:valpri}.
  %\item[] \textbf{Output:} See Definition~\ref{def:valpri}.
  \end{asparaitem}
\end{definition}

\subsection{Unlinkability}

Sketch of the definition of unlinkability. Note that we require the whole path to be composed by honest nodes. I do not know how to instantiate it otherwise. I am not sure if it is even possible, maybe with onion routing but we have to discuss the exact properties.

\begin{definition}[Unlinkability]\label{def:unlink}
  We say that a scheme achieves \emph{unlinkability} if for all $\lambda
  \in \NN$ and for all probabilistic-polynomial time adversaries
  $\adv$ there exists a negligible function such that the success
  probability of $\adv$ in the following experiment is negligibly
  close to $\frac{1}{2}$.
  \begin{asparaitem}
  %\item[] \textbf{Setup \& Phase 1:} See Definition~\ref{def:valpri}.
  %\item[] \textbf{Phase 1:} See Definition~\ref{def:valpri}.
  \item[] \textbf{Challenge:} The adversary outputs a tuple $(C=(c_1^*, \dots, c_n^*), v,
    i)$.  For such a tuple to be admissible we
    require that $(c_1^*, \dots, c_n^*) \in \mathcal{H}^n$. The challenger than flips a bit $b \in \{ 0,1\}$ and executes either $\pay(C, v)$ if $b=1$, or $\pay((c_1^*, \dots, c_i^*),v)$ and $\pay((c_i^*,\dots, c_n^*),v)$ otherwise. If any of the transactions was not successful, the challenger aborts.
  %\item[] \textbf{Phase 2 \& Output:} See Definition~\ref{def:valpri}.
  %\item[] \textbf{Output:} See Definition~\ref{def:valpri}.
  \end{asparaitem}
\end{definition}

\subsection{Atomicity}

Sketch of the definition of atomicity.

\begin{definition}[Atomicity]\label{def:atom}
  We say that a scheme achieves \emph{atomicity} if for all $\lambda
  \in \NN$ and for all probabilistic-polynomial time adversaries
  $\adv$ there exists a negligible function such that the success
  probability of $\adv$ in the following experiment is negligibly
  close to $\frac{1}{2}$.
  \begin{asparaitem}
  %\item[] \textbf{Setup \& Phase 1:} See Definition~\ref{def:valpri}.
  %\item[] \textbf{Phase 1:} See Definition~\ref{def:valpri}.
  \item[] \textbf{Challenge:} The adversary outputs a tuple $(C=(c_1^*, \dots, c_n^*), v,
    i)$. The challenger then executes $\pay(C, v)$ in interaction with the adversary, impersonating the honest clients. 
  %\item[] \textbf{Phase 2 \& Output:} See Definition~\ref{def:valpri}.
  \item[] \textbf{Output:} Let $\Delta_{c_i^*}$ denote the sum of all the values of the links adjacent to the client $c_i^*$ before the operation and $\Delta_{c_i^*}'$ the same variable after the transaction. The challenger checks whether $\forall c_i^* \in \mathcal{H}: \Delta_{c_i^*} = \Delta_{c_i^*}'$. If this condition is not verified the challenger returns $1$. Additionally, if $(c_1^*, c_n^*) \in \mathcal{H}$ then the challenger verifies whether $\Delta_{c_1^*} = \Delta_{c_1^*}'$ or $(\Delta_{c_1^*} = \Delta_{c_1^*}' - v \land \Delta_{c_n^*} = \Delta_{c_n^*}' +v)$. If neither of these conditions hold the challenger returns $1$, otherwise it outputs $0$.
  \end{asparaitem}
\end{definition}

\subsection{Proof of Theorem~\ref{thm:valpri}}
\begin{proof}
  We observe that, if there exists an $i \in [m]$ such that $c_i^* \in
  \mathcal{C}$, then the two challenge values $\val_0$ and $\val_1$ have to
  be the same and therefore the two experiments are
  identical. Therefore we consider without loss of generality that for
  all $i \in [m]: c_i^* \in \mathcal{H}$. Since the communication
  between honest clients happens through secure and authenticated
  channels, the indistinguishability argument is straighforward.
\end{proof}


\subsection{Proof of Theorem~\ref{thm:testpri}}

\begin{proof}
  Assume towards contradiction that there exists an adversary $\adv$
  that wins the test privacy experiment with non-negligible advantage
  $\epsilon(\lambda)$. We discuss the four cases described in
  Definition~\ref{def:testpri} separately and we argue why in each
  case $\epsilon(\lambda)$ can be bound to a negligible function.

  \paragraph{$(\sender, \receiver) \in \mathcal{C}^2:$} We modify the simulation of the
  experiment as follows: On input $((c_1, \dots, c_n), r_0, \val')$ by
  $\adv$ (on behalf of $\sender$) we first check whether $\val'$ is equal to
  the challenge $\val$ and abort if this condition is not met. Then
  for all $j \in [m]$ and for all $i \in [n]$ we fix:
  \[
  r_j||\uid_{j+1} := \{ \dec(\dk_j, c_i) \mid \dec(\dk_j, c_i) \ne \bot\}
  \]
  in case this is satisfied by more than one $c_i$, we take the value
  of $\dec(\dk_j, c_i)$ with the highest $i$. In case there exists
  some $\uid_j \in \mathcal{C}$ (except for the receiver $\receiver$),
  we abort the simulation. Then we simulate the communication between
  honest nodes with random messages. Finally we provide the receiver
  $\receiver$ with the the tuple $((c_1, \dots, c_n), s)$ where $s$ is
  defined as:
  \[s := 
    \begin{cases} 
      \bigoplus_{j \in \{ 0, \dots, m\}} r_j &\mbox{if } \mathrm{min}\{ w_i^0\}_{i\in[m]} \ge \val \\
      s \gets \{ 0,1\}^\lambda & \mbox{if }\mathrm{min}\{ w_i^0\}_{i\in[m]} < \val 
    \end{cases} 
  \]
  The simulation is clearly efficient and it reproduces exactly the
  inputs that $\adv$ is expecting in the original experiment for
  $b=0$. We observe that by the non-triviality condition of the game
  it holds that
  \[
  \mathrm{min}\{ w_i^0\}_{i\in[m]} \ge \val \implies \mathrm{min}\{ w_i^1\}_{i\in[m]} \ge \val,
  \]
  and that
  \[
  \mathrm{min}\{ w_i^0\}_{i\in[m]} < \val \implies \mathrm{min}\{ w_i^1\}_{i\in[m]} < \val.
  \]
  This implies that the simulation for the case of $b=1$ is identical.
  What is left to be shown is that the simulation correctly reproduces
  the communication among honest nodes to the eyes of the
  adversary. Since we assumed the existence of secure and
  authenticated channels between pairs of nodes, the argument is
  trivial and therefore is omitted. We conclude that, for the case
  $(\sender, \receiver) \in \mathcal{C}^2$, the function $\epsilon(\lambda)$ must be
  negligible.

  \paragraph{$\sender \in \mathcal{C}:$} The argument is identical to
  the one described above, except that we do not provide the adversary
  with the output of the receiver. It is easy to see that even in this
  case the advantage of the adversary must be negligible.

  \paragraph{$\receiver \in \mathcal{C}:$} The argument is exactly the
  same as the first case except that the first message of the
  challenge $\test$ query is honestly generated by the challenger, who
  executes $\test((c_1^*, \dots, c_m^*), \val)$. As before, if
  $(c_1^*, \dots, c_m^*) \not\in \mathcal{H}^m$ the challenger
  aborts. The indistinguishability argument follows along the same
  lines.

  \paragraph{$(\sender, \receiver) \in \mathcal{H}^2:$} We modify the
  game for $\test$ privacy thorugh a serie of hybird experiments
  $(H_0, \dots, H_m)$ that we define as follows:
  \begin{itemize}
  \item[$H_0$:] Resembles the game as described in Definition~\ref{def:testpri}.
  \item[$\dots$]
  \item[$H_j$:] If $c_j^* \in \mathcal{C}$, then $H_j$ is defined as
    $H_{j-1}$. Otherwise $H_j$ is a modification of $H_{j-1}$, where
    the ciphertext $c_j$ of the challenge $\test$ query is generated
    by the challenger as $\enc(\ek_{c_j^*},0)$. The user $c_j^*$ is
    simulated by the challenger as specified in
    Figure~\ref{fig:test-operations} except if the user has to decrypt
    $c_j$. In that case the values $r_j||\uid_{j+1}$ are recovered by
    the internal state of the sender (which is anyway simulated by the
    challenger).
  \end{itemize}
  We prove that $H_0$ is indistinguishable from $H_m$ to the eyes of
  the adversary via a standard hybrid argument. Assume towards
  contradiction that there exists an adversary $\adv'$ that can
  distinguish between $H_0$ and $H_m$ with non-negligible probability
  $\phi(\lambda)$. Then it must be the case that there exists a $0 < j
  \le m$ such that $\adv'$ can distinguish $H_{j-1}$ from $H_{j}$ with
  the same probability. We can construct the following reduction
  against the chosen-ciphertext security of $\Pi^\mathsf{PKE}$
  (see~\cite{cca} for a formal definition):
  \begin{itemize}
  \item[$\red(1^\lambda, \ek)$] Let $q$ be the number of clients
    spawned by $\adv'$, on input $(1^\lambda, \ek)$ the reduction
    samples a random $j \in [m]$ and a random $k \in [q]$ and
    simulates the experiment as defined in $H_j$, assigning $\ek$ as
    the public key of the $k$-th client. If the adversary tries to
    corrupt such a client, the reduction aborts. Any decryption that
    the $k$-th client must perform is simulated by querying the
    decryption oracle offered by the challenger. In the challenge
    phase, the reduction outputs the tuple $(r_j||\uid_{j+1}, 0)$ and
    receives in response the ciphertext $c'$. $\red$ then sets $c_j =
    c'$ and continues with the simulation as specified in $H_j$. At
    some point of the execution, $\adv'$ returns a bit $b'$ that the
    reduction outputs.
  \end{itemize}
  The algorithm $\red$ is clearly efficieny. Assume for the moment
  that the reduction correctly guesses the values of $j$ and $k$. We
  observe that when $c' = \enc(\ek, r_j||\uid_{j+1})$, then the
  reduction simulates the inputs that $\adv'$ is expecting in
  $H_{j-1}$, therefore we have that
  \[
  \prob{1 \gets \red \mid c' = \enc(\ek, r_j||\uid_{j+1})} = \prob{1
    \gets \adv' \mid H_{j-1}}.
  \]
  On the other hand, when $c' = \enc(\ek, 0)$ then the reduction
  simulates the input that $\adv'$ is expecting in $H_j$. Thus we can
  rewrite
    \[
  \prob{1 \gets \red \mid c' = \enc(\ek, 0)} = \prob{1
    \gets \adv' \mid H_{j}}.
  \]
  By the initial assumption we have that, when $\red$ correctly
  samples $j$ and $k$, it holds that
  \[ \left|
  \begin{array}{l}
    \prob{1 \gets \red \mid c' = \enc(\ek, r_j||\uid_{j+1})} -\\
    \quad \prob{1 \gets \red \mid c' = \enc(\ek, 0)}
  \end{array} 
  \right|\ge \phi(\lambda).
  \]
  Since $\red$ correctly samples $j$ with probability at least
  $\frac{1}{m}$ and $k$ with probability $\frac{1}{q}$, we have that
  the advantage of $\red$ is at least $\frac{\phi(\lambda)}{m \cdot
    q}$.  By the chosen ciphertext security of $\Pi^\mathsf{PKE}$, it follows
  that $\phi(\lambda)$ must be a negligible function. This implies
  that, for all $\adv: H_0 \approx H_m$. We now observe that the
  outputs seen by the adversary in $H_m$ are indentically distributed
  for both the cases $b=0$ and $b=1$: Since, for all $j$, $c_j$ is no longer an
  encryption of $r_j$, then $r \oplus r_j$ is a string uniformly
  distributed in $\{0,1\}^\lambda$. We can conclude that the advantage
  of the adversary $\epsilon(\lambda)$ must be a negligible
  function. This concludes our proof.
\end{proof}



\section{Proof of Theorem~\ref{thm:anon}}

\begin{proof}
  Assume towards contradiction that there exists an adversary $\adv$
  that wins the anonymity experiment with non-negligible advantage
  $\epsilon(\lambda)$. We graudually modify the simulation thorugh a
  serie of hybird experiments $(H_0, \dots, H_m)$ that we define as
  follows:
  \begin{itemize}
  \item[$H_0$:] Resembles the game as described in Definition~\ref{def:anon}.
  \item[$\dots$]
  \item[$H_j$:] If either $c_{j-1}^*$, $c_{j}^*$, or $c_{j+1}^*$ are
    corrupted, then $H_j$ is defined as $H_{j-1}$. Otherwise $H_j$ is
    a modification of $H_{j-1}$, where the ciphertext $c_j$ of the
    challenge $\test$ query is generated by the challenger as
    $\enc(\ek',r_j||\uid_{j+1})$, for a fresh $\ek'$. The user $c_j^*$
    is simulated by the challenger as specified in
    Figure~\ref{fig:test-operations} except that if one ciphertext in
    the vector $(c_1, \dots, c_n)$ is $c_j$, the user sets
    $r_j||\uid_{j+1}$ according to the internal state of the challenger
    (i.e., recovers $r_j||\uid_{j+1}$ without decrypting $c_j$).
  \end{itemize}
  We prove indistinguishability of neighbouring experiments via a
  standard hybrid argument. Assume towards contradiction that there
  exists an adversary $\adv'$ that can distinguish between $H_0$ and
  $H_m$ with non-negligible probability $\phi(\lambda)$. Then it must
  be the case that there exists a $0 < j \le m$ such that $\adv'$ can
  distinguish $H_{j-1}$ from $H_{j}$ with the same probability. We can
  construct the following reduction against the key-privacy of
  $\Pi^\mathsf{PKE}$ (see~\cite{keyprivacy} for a formal definition):
  \begin{itemize}
  \item[$\red(1^\lambda, \ek_0, \ek_1)$] Let $q$ be the number of
    clients spawned by $\adv'$, on input $(1^\lambda, \ek_0, \ek_1)$
    the reduction samples a random $j \in [m]$ and a random $k \in
    [q]$ and simulates the experiment as defined in $H_j$, assigning
    $\ek_0$ as the public key of the $k$-th client. Whenever the
    reduction must simulate a decryption of beahalf of this client it
    queries the decryption oracle for $\ek_0$ provided by the
    challenger. If the adversary tries to corrupt the client with key
    $\ek_0$, the reduction aborts. In the challenge phase, the
    reduction outputs the tuple $(r_j||\uid_{j+1})$ and receives in
    response the ciphertext $c'$. $\red$ then sets $c_j = c'$ and
    continues with the simulation as specified in $H_j$. At some point
    of the execution, $\adv'$ returns a bit $b'$ that the reduction
    outputs to the challenger and interrupts the execution of $\adv'$.
  \end{itemize}
  The algorithm $\red$ is obviously efficieny. Assume for the moment
  that the reduction correctly guesses the values of $j$ and $k$. We
  observe that when $c' = \enc(\ek_0, r_j||\uid_{j+1})$, then the
  reduction simulates the inputs that $\adv'$ is expecting in
  $H_{j-1}$, therefore we have that
  \[
  \prob{1 \gets \red \mid c' = \enc(\ek_0, r_j||\uid_{j+1})} = \prob{1
    \gets \adv' \mid H_{j-1}}.
  \]
  On the other hand, when $c' = \enc(\ek_1,r_j||\uid_{j+1})$ then the reduction
  simulates the input that $\adv'$ is expecting in $H_j$. Thus we can
  rewrite
    \[
  \prob{1 \gets \red \mid c' = \enc(\ek_1, r_j||\uid_{j+1})} = \prob{1
    \gets \adv' \mid H_{j}}.
  \]
  By the initial assumption we have that, when $\red$ correctly
  samples $j$ and $k$, it holds that
  \[ \left|
  \begin{array}{l}
    \prob{1 \gets \red \mid c' = \enc(\ek_0, r_j||\uid_{j+1})} -\\
    \quad \prob{1 \gets \red \mid c' = \enc(\ek_1, r_j||\uid_{j+1})}
  \end{array} 
  \right|\ge \phi(\lambda).
  \]
  Since $\red$ correctly samples $j$ with probability at least
  $\frac{1}{m}$ and $k$ with probability $\frac{1}{q}$, we have that
  the advantage of $\red$ is at least $\frac{\phi(\lambda)}{m \cdot
    q}$.  By the chosen ciphertext security of $\Pi^\mathsf{PKE}$, it
  follows that $\phi(\lambda)$ must be a negligible function. This
  implies that the experiment $H_0$ and $H_m$ are indistinguishable to
  the eyes of any adversary. Now we further modify the experiment
  following another series of hybrids $(H_m, \dots, H_{2m})$ that we
  define as follows:
  \begin{itemize}
  \item[$H_m$:] Is defined as above.
  \item[$\dots$]
  \item[$H_{m+j}$:] If $c_j^* \in \mathcal{C}$, then $H_{m+j}$ is
    defined as $H_{m+j-1}$. Otherwise $H_{m+j}$ is a modification of
    $H_{m+j-1}$, where the ciphertext $c_j$ of the challenge $\test$
    query is generated by the challenger as an encryption of $0$.
  \end{itemize}
  The indistinguishability argument follows along the same lines as
  the one formalized for the proof of Theorem~\ref{thm:testpri}. This
  implies that the experiments $H_0$ and $H_{2m}$ are computationally
  indistinguishable to the eyes of any efficient adversary $\adv$. We
  now observe that, due to the non-triviality requirements of
  Definition~\ref{def:anon} the simulation of $H_{2m}$ is identical
  for both cases $b=0$ and $b=1$: Note that all of the ciphertexts of
  the challenge set $(c_1, \dots, c_n)$, that are encrypted for
  non-corrupted clients, are defined as encryptions of
  $0$. Furthermore, the simulation of $H_{2m}$ defines the ciphertexts
  of users without links with corrupted nodes, as encryptions under
  freshly sampled public keys. Since the users neighbouring the
  adversary are required to be the same in both challege sets, we have
  that the vector $(c_1, \dots, c_n)$ is identically distributed for
  both cases. It follows that $\epsilon(\lambda)$ must be a negligible
  function. This concludes our proof.
\end{proof}

\subsection{Privacy and Concurrency}

Since we formalize the privacy properties as game-based
indistinguishability notions, we prove our construction secure only in
the stand-alone model. Reasoning about security in concurrent settings
is in general possible in the Universal Composability (UC) framework
of Canetti~\cite{CanettiUC}. This however requires the formalization
of an ideal functionality of the interactions among users, which is
highly non-trivial, especially for complex system like ours. For
simplicity and readability, we concrentrate on the simpler (and
arguably more intuitive) privacy in the stand-alone model and we leave
the formalization of a UC definition for Payment Channel Networks as
an interesting future work. We do however remark that our construction
is built on top of simple and \emph{non interactive} cryptographic
primitives. For this reason we strongly belive that our scheme can be
proven secure in presence of concurrent executions with minor
modifications.



